When Lawvere meets Peirce: an equational presentation of boolean hyperdoctrines

Fo-bicategories are a categorification of Peirce's calculus of relations. Notably, their laws provide a proof system for first-order logic that is both purely equational and complete. This paper illustrates a correspondence between fo-bicategories and Lawvere's hyperdoctrines. To streamline our proof, we introduce peircean bicategories, which offer a more succinct characterization of fo-bicategories.

==> tikz/proofs/deductionTheorem/seqMinus.tex <==
\[
\begin{array}{rcl}
    \tikzfig{cPerId} 
    &\stackrel{\eqref{ax:comPlusLaxNat}}{\syninclusionT{\T{T}}}&
    \tikzfig{cPerCperId} 
    \stackrel{\text{Ind. hyp.}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, -0.625) {};
            \node [style=none] (112) at (-3.75, 0.125) {};
            \node [style=none] (113) at (-3.75, -1.375) {};
            \node [style=none] (114) at (-0.25, -1.375) {};
            \node [style=none] (115) at (-0.25, 0.125) {};
            \node [style=none] (121) at (-0.25, -0.625) {};
            \node [{boxStyle/+}] (122) at (-2.75, -0.625) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (-1.25, -0.625) {${a_1}$};
            \node [style=none] (124) at (-4, 1.625) {};
            \node [style=none] (125) at (-4, -1.625) {};
            \node [style=none] (126) at (0, -1.625) {};
            \node [style=none] (127) at (0, 1.625) {};
            \node [style=none] (128) at (-4, -0.625) {};
            \node [style=none] (138) at (0, -0.625) {};
            \node [style={boxStyle/+}] (139) at (-1.25, 0.875) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [style={wStyle/+}] (81.center) to (128.center);
            \draw [style={wStyle/+}] (121.center) to (138.center);
        \end{pgfonlayer}
    \end{tikzpicture}      
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, -0.875) {};
            \node [style=none] (112) at (-3.75, -0.125) {};
            \node [style=none] (113) at (-3.75, -1.625) {};
            \node [style=none] (114) at (-0.25, -1.625) {};
            \node [style=none] (115) at (-0.25, -0.125) {};
            \node [style=none] (121) at (-0.25, -0.875) {};
            \node [{boxStyle/+}] (122) at (-2.75, -0.875) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (-1.25, -0.875) {${a_1}$};
            \node [style=none] (124) at (-4, 1.875) {};
            \node [style=none] (125) at (-4, -1.875) {};
            \node [style=none] (126) at (0, -1.875) {};
            \node [style=none] (127) at (0, 1.875) {};
            \node [style=none] (128) at (-4, -0.875) {};
            \node [style=none] (138) at (0, -0.875) {};
            \node [style={boxStyle/+}] (139) at (-1.25, 0.875) {$c$};
            \node [style=none] (140) at (-3.75, 1.625) {};
            \node [style=none] (141) at (-3.75, 0.125) {};
            \node [style=none] (142) at (-0.25, 0.125) {};
            \node [style=none] (143) at (-0.25, 1.625) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{bgStyle/-}] (142.center)
                 to (141.center)
                 to (140.center)
                 to (143.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [style={wStyle/+}] (81.center) to (128.center);
            \draw [style={wStyle/+}] (121.center) to (138.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \stackrel{\eqref{ax:linStrn1}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.375, -0.875) {};
            \node [style=none] (112) at (-0.375, 1.625) {};
            \node [style=none] (113) at (-0.375, -1.625) {};
            \node [style=none] (114) at (-2.125, -1.625) {};
            \node [style=none] (115) at (-2.125, 1.625) {};
            \node [{boxOpStyle/-}] (122) at (-1.25, -0.875) {${a_1}$};
            \node [{boxStyle/+}] (123) at (-3.125, -0.875) {$b_1$};
            \node [style=none] (124) at (-0.125, 1.875) {};
            \node [style=none] (125) at (-0.125, -1.875) {};
            \node [style=none] (126) at (-4.125, -1.875) {};
            \node [style=none] (127) at (-4.125, 1.875) {};
            \node [style=none] (128) at (-0.125, -0.875) {};
            \node [style=none] (138) at (-4.125, -0.875) {};
            \node [style={boxStyle/+}] (139) at (-1.25, 0.875) {$c$};
            \node [style=none] (140) at (-2.125, -0.875) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [style={wStyle/+}] (122) to (140.center);
            \draw [style={wStyle/-}] (81.center) to (128.center);
            \draw [style={wStyle/-}] (140.center) to (123);
            \draw [style={wStyle/-}] (123) to (138.center);
        \end{pgfonlayer}
    \end{tikzpicture}     
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.125, -0.375) {};
            \node [style=none] (112) at (-0.125, 1.125) {};
            \node [style=none] (113) at (-0.125, -1.125) {};
            \node [style=none] (114) at (-3.375, -1.125) {};
            \node [style=none] (115) at (-3.375, 1.125) {};
            \node [{boxOpStyle/-}] (122) at (-1, -0.375) {${a_1}$};
            \node [{boxStyle/+}] (123) at (-4.375, -0.375) {$b_1$};
            \node [style=none] (124) at (0.125, 1.375) {};
            \node [style=none] (125) at (0.125, -1.375) {};
            \node [style=none] (126) at (-5.375, -1.375) {};
            \node [style=none] (127) at (-5.375, 1.375) {};
            \node [style=none] (128) at (0.125, -0.375) {};
            \node [style=none] (138) at (-5.375, -0.375) {};
            \node [style={boxStyle/+}] (139) at (-2.4, 0.375) {$c$};
            \node [style=none] (140) at (-3.375, -0.375) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/+}] (122) to (140.center);
            \draw [style={wStyle/-}] (81.center) to (128.center);
            \draw [style={wStyle/-}] (140.center) to (123);
            \draw [style={wStyle/-}] (123) to (138.center);
            \draw [style={wStyle/+}] (81.center) to (122);
        \end{pgfonlayer}
    \end{tikzpicture}  \\[20pt]
    &\!\!\! \stackrel{\text{Ind. hyp.}}{\syninclusionT{\T{T}}} \!\!\!&
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (112) at (1.4, 0.75) {};
            \node [style=none] (113) at (1.4, -0.75) {};
            \node [style=none] (114) at (-2, -0.75) {};
            \node [style=none] (115) at (-2, 0.75) {};
            \node [{boxOpStyle/-}] (122) at (2.25, 0) {${a_1}$};
            \node [{boxOpStyle/-}] (123) at (0.5, 0) {${a_2}$};
            \node [style=none] (124) at (3, 1) {};
            \node [style=none] (125) at (3, -1) {};
            \node [style=none] (126) at (-2.25, -1) {};
            \node [style=none] (127) at (-2.25, 1) {};
            \node [style=none] (128) at (3, 0) {};
            \node [style=none] (135) at (-2.25, 0) {};
            \node [{boxStyle/+}] (136) at (-1.05, 0) {$b_2$};
            \node [{boxStyle/+}] (137) at (-3.25, 0) {$b_1$};
            \node [style=none] (138) at (3.25, 1.25) {};
            \node [style=none] (139) at (3.25, -1.25) {};
            \node [style=none] (140) at (-4.25, -1.25) {};
            \node [style=none] (141) at (-4.25, 1.25) {};
            \node [style=none] (142) at (-4.25, 0) {};
            \node [style=none] (143) at (3.25, 0) {};
            \node [style=none] (144) at (1.4, 0) {};
            \node [style=none] (145) at (-2, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (140.center)
                 to (139.center)
                 to (138.center)
                 to (141.center)
                 to cycle;
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/-}] (135.center) to (137);
            \draw [style={wStyle/-}] (137) to (142.center);
            \draw [style={wStyle/-}] (123) to (136);
            \draw [style={wStyle/-}] (143.center) to (128.center);
            \draw [style={wStyle/+}] (128.center) to (122);
            \draw [style={wStyle/+}] (144.center) to (122);
            \draw [style={wStyle/-}] (123) to (144.center);
            \draw [style={wStyle/+}] (135.center) to (145.center);
            \draw [style={wStyle/-}] (136) to (145.center);
        \end{pgfonlayer}
    \end{tikzpicture}              
    \stackrel{\eqref{ax:rightLinDistr}}{\syninclusionT{\T{T}}}   
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (3, 0) {};
            \node [style=none] (112) at (3, 0.75) {};
            \node [style=none] (113) at (3, -0.75) {};
            \node [style=none] (114) at (-0.5, -0.75) {};
            \node [style=none] (115) at (-0.5, 0.75) {};
            \node [style=none] (121) at (-0.5, 0) {};
            \node [{boxOpStyle/-}] (122) at (2, 0) {${a_2}$};
            \node [{boxOpStyle/-}] (123) at (0.5, 0) {${a_1}$};
            \node [style=none] (124) at (3.25, 1) {};
            \node [style=none] (125) at (3.25, -1) {};
            \node [style=none] (126) at (-4, -1) {};
            \node [style=none] (127) at (-4, 1) {};
            \node [style=none] (128) at (3.25, 0) {};
            \node [{boxStyle/+}] (136) at (-1.5, 0) {$b_2$};
            \node [{boxStyle/+}] (137) at (-3, 0) {$b_1$};
            \node [style=none] (138) at (-4, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/-}] (128.center) to (81.center);
            \draw [style={wStyle/-}] (121.center) to (136);
            \draw [style={wStyle/-}] (136) to (137);
            \draw [style={wStyle/-}] (137) to (138.center);
            \draw [style={wStyle/+}] (123) to (121.center);
            \draw [style={wStyle/+}] (123) to (122);
            \draw [style={wStyle/+}] (122) to (81.center);
        \end{pgfonlayer}
    \end{tikzpicture}        
\end{array}
\]

==> tikz/proofs/deductionTheorem/seqPlus.tex <==
\[
\begin{array}{rcl}
    \tikzfig{cPerId} 
    &\stackrel{\eqref{ax:comPlusLaxNat}}{\syninclusionT{\T{T}}}&
    \tikzfig{cPerCperId} 
    \stackrel{\text{Ind. hyp.}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, -0.625) {};
            \node [style=none] (112) at (-3.75, 0.125) {};
            \node [style=none] (113) at (-3.75, -1.375) {};
            \node [style=none] (114) at (-0.25, -1.375) {};
            \node [style=none] (115) at (-0.25, 0.125) {};
            \node [style=none] (121) at (-0.25, -0.625) {};
            \node [{boxStyle/+}] (122) at (-2.75, -0.625) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (-1.25, -0.625) {$a_1$};
            \node [style=none] (124) at (-4, 1.625) {};
            \node [style=none] (125) at (-4, -1.625) {};
            \node [style=none] (126) at (0, -1.625) {};
            \node [style=none] (127) at (0, 1.625) {};
            \node [style=none] (128) at (-4, -0.625) {};
            \node [style=none] (138) at (0, -0.625) {};
            \node [style={boxStyle/+}] (139) at (-2.75, 0.875) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [style={wStyle/+}] (81.center) to (128.center);
            \draw [style={wStyle/+}] (121.center) to (138.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, -0.875) {};
            \node [style=none] (112) at (-3.75, -0.125) {};
            \node [style=none] (113) at (-3.75, -1.625) {};
            \node [style=none] (114) at (-0.25, -1.625) {};
            \node [style=none] (115) at (-0.25, -0.125) {};
            \node [style=none] (121) at (-0.25, -0.875) {};
            \node [{boxStyle/+}] (122) at (-2.75, -0.875) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (-1.25, -0.875) {$a_1$};
            \node [style=none] (124) at (-4, 1.875) {};
            \node [style=none] (125) at (-4, -1.875) {};
            \node [style=none] (126) at (0, -1.875) {};
            \node [style=none] (127) at (0, 1.875) {};
            \node [style=none] (128) at (-4, -0.875) {};
            \node [style=none] (138) at (0, -0.875) {};
            \node [style={boxStyle/+}] (139) at (-2.75, 0.875) {$c$};
            \node [style=none] (140) at (-3.75, 1.625) {};
            \node [style=none] (141) at (-3.75, 0.125) {};
            \node [style=none] (142) at (-0.25, 0.125) {};
            \node [style=none] (143) at (-0.25, 1.625) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{bgStyle/-}] (142.center)
                 to (141.center)
                 to (140.center)
                 to (143.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [style={wStyle/+}] (81.center) to (128.center);
            \draw [style={wStyle/+}] (121.center) to (138.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \stackrel{\eqref{ax:linStrn2}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.875, -0.875) {};
            \node [style=none] (112) at (-3.875, 1.625) {};
            \node [style=none] (113) at (-3.875, -1.625) {};
            \node [style=none] (114) at (-2.125, -1.625) {};
            \node [style=none] (115) at (-2.125, 1.625) {};
            \node [{boxStyle/+}] (122) at (-3, -0.875) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (-1.125, -0.875) {$a_1$};
            \node [style=none] (124) at (-4.125, 1.875) {};
            \node [style=none] (125) at (-4.125, -1.875) {};
            \node [style=none] (126) at (-0.125, -1.875) {};
            \node [style=none] (127) at (-0.125, 1.875) {};
            \node [style=none] (128) at (-4.125, -0.875) {};
            \node [style=none] (138) at (-0.125, -0.875) {};
            \node [style={boxStyle/+}] (139) at (-3, 0.875) {$c$};
            \node [style=none] (140) at (-2.125, -0.875) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [style={wStyle/+}] (122) to (140.center);
            \draw [style={wStyle/-}] (81.center) to (128.center);
            \draw [style={wStyle/-}] (140.center) to (123);
            \draw [style={wStyle/-}] (123) to (138.center);
        \end{pgfonlayer}
    \end{tikzpicture} 
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-5.125, -0.375) {};
            \node [style=none] (112) at (-5.125, 1.125) {};
            \node [style=none] (113) at (-5.125, -1.125) {};
            \node [style=none] (114) at (-1.875, -1.125) {};
            \node [style=none] (115) at (-1.875, 1.125) {};
            \node [{boxStyle/+}] (122) at (-4.25, -0.375) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (-0.875, -0.375) {$a_1$};
            \node [style=none] (124) at (-5.375, 1.375) {};
            \node [style=none] (125) at (-5.375, -1.375) {};
            \node [style=none] (126) at (0.125, -1.375) {};
            \node [style=none] (127) at (0.125, 1.375) {};
            \node [style=none] (128) at (-5.375, -0.375) {};
            \node [style=none] (138) at (0.125, -0.375) {};
            \node [style={boxStyle/+}] (139) at (-2.85, 0.375) {$c$};
            \node [style=none] (140) at (-1.875, -0.375) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/+}] (122) to (140.center);
            \draw [style={wStyle/-}] (81.center) to (128.center);
            \draw [style={wStyle/-}] (140.center) to (123);
            \draw [style={wStyle/-}] (123) to (138.center);
            \draw [style={wStyle/+}] (81.center) to (122);
        \end{pgfonlayer}
    \end{tikzpicture} \\[20pt]
    &\!\!\! \stackrel{\text{Ind. hyp.}}{\syninclusionT{\T{T}}} \!\!\!&
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (112) at (-2.5, 0.75) {};
            \node [style=none] (113) at (-2.5, -0.75) {};
            \node [style=none] (114) at (1, -0.75) {};
            \node [style=none] (115) at (1, 0.75) {};
            \node [{boxStyle/+}] (122) at (-3.25, 0) {$b_1$};
            \node [{boxStyle/+}] (123) at (-1.5, 0) {$b_2$};
            \node [style=none] (124) at (-4, 1) {};
            \node [style=none] (125) at (-4, -1) {};
            \node [style=none] (126) at (1.25, -1) {};
            \node [style=none] (127) at (1.25, 1) {};
            \node [style=none] (128) at (-4, 0) {};
            \node [style=none] (135) at (1.25, 0) {};
            \node [{boxOpStyle/-}] (136) at (0.05, 0) {$a_2$};
            \node [{boxOpStyle/-}] (137) at (2.25, 0) {$a_1$};
            \node [style=none] (138) at (-4.25, 1.25) {};
            \node [style=none] (139) at (-4.25, -1.25) {};
            \node [style=none] (140) at (3.25, -1.25) {};
            \node [style=none] (141) at (3.25, 1.25) {};
            \node [style=none] (142) at (3.25, 0) {};
            \node [style=none] (143) at (-4.25, 0) {};
            \node [style=none] (144) at (-2.5, 0) {};
            \node [style=none] (145) at (1, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (140.center)
                 to (139.center)
                 to (138.center)
                 to (141.center)
                 to cycle;
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/-}] (135.center) to (137);
            \draw [style={wStyle/-}] (137) to (142.center);
            \draw [style={wStyle/-}] (123) to (136);
            \draw [style={wStyle/-}] (143.center) to (128.center);
            \draw [style={wStyle/+}] (128.center) to (122);
            \draw [style={wStyle/+}] (144.center) to (122);
            \draw [style={wStyle/-}] (123) to (144.center);
            \draw [style={wStyle/-}] (136) to (145.center);
            \draw [style={wStyle/+}] (145.center) to (135.center);
        \end{pgfonlayer}
    \end{tikzpicture}         
    \stackrel{\eqref{ax:leftLinDistr}}{\syninclusionT{\T{T}}}   
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, 0) {};
            \node [style=none] (112) at (-3.75, 0.75) {};
            \node [style=none] (113) at (-3.75, -0.75) {};
            \node [style=none] (114) at (-0.25, -0.75) {};
            \node [style=none] (115) at (-0.25, 0.75) {};
            \node [style=none] (121) at (-0.25, 0) {};
            \node [{boxStyle/+}] (122) at (-2.75, 0) {$b_1$};
            \node [{boxStyle/+}] (123) at (-1.25, 0) {$b_2$};
            \node [style=none] (124) at (-4, 1) {};
            \node [style=none] (125) at (-4, -1) {};
            \node [style=none] (126) at (3.25, -1) {};
            \node [style=none] (127) at (3.25, 1) {};
            \node [style=none] (128) at (-4, 0) {};
            \node [{boxOpStyle/-}] (136) at (0.75, 0) {$a_2$};
            \node [{boxOpStyle/-}] (137) at (2.25, 0) {$a_1$};
            \node [style=none] (138) at (3.25, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/-}] (128.center) to (81.center);
            \draw [style={wStyle/-}] (121.center) to (136);
            \draw [style={wStyle/-}] (136) to (137);
            \draw [style={wStyle/-}] (137) to (138.center);
            \draw [style={wStyle/+}] (123) to (121.center);
            \draw [style={wStyle/+}] (123) to (122);
            \draw [style={wStyle/+}] (122) to (81.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
\end{array}
\]

==> tikz/proofs/deductionTheorem/tensorMinus.tex <==
\[
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, 0) {};
            \node [style=none] (112) at (-0.75, 1.25) {};
            \node [style=none] (113) at (-0.75, -1) {};
            \node [style=none] (114) at (0.75, -1) {};
            \node [style=none] (115) at (0.75, 1.25) {};
            \node [style=none] (121) at (0.75, 0) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (0, 0.65) {$c$};
            \node [style=none] (123) at (-0.75, -0.5) {};
            \node [style=none] (124) at (0.75, -0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
            \draw [{wStyle/+}] (123.center) to (124.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \stackrel{\eqref{ax:comPlusLaxNat}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, -0.675) {};
            \node [style=none] (112) at (-0.75, 1.575) {};
            \node [style=none] (113) at (-0.75, -1.675) {};
            \node [style=none] (114) at (0.75, -1.675) {};
            \node [style=none] (115) at (0.75, 1.575) {};
            \node [style=none] (121) at (0.75, -0.675) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (0, -0.025) {$c$};
            \node [style=none] (123) at (-0.75, -1.175) {};
            \node [style=none] (124) at (0.75, -1.175) {};
            \node [style={boxStyle/+}, scale=0.8] (125) at (0, 0.975) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
            \draw [{wStyle/+}] (123.center) to (124.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, 0.325) {};
            \node [style=none] (112) at (-0.75, 1.575) {};
            \node [style=none] (113) at (-0.75, -1.675) {};
            \node [style=none] (114) at (0.75, -1.675) {};
            \node [style=none] (115) at (0.75, 1.575) {};
            \node [style=none] (121) at (0.75, 0.325) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (0, -0.525) {$c$};
            \node [style=none] (123) at (-0.75, -1.175) {};
            \node [style=none] (124) at (0.75, -1.175) {};
            \node [style={boxStyle/+}, scale=0.8] (125) at (0, 0.975) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
            \draw [{wStyle/+}] (123.center) to (124.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \stackrel{\text{Ind. hyp.}}{\synequivalenceT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-1.75, 0.875) {};
            \node [style=none] (112) at (-1.75, 1.625) {};
            \node [style=none] (113) at (-1.75, 0.125) {};
            \node [style=none] (114) at (1.75, 0.125) {};
            \node [style=none] (115) at (1.75, 1.625) {};
            \node [style=none] (121) at (1.75, 0.875) {};
            \node [{boxStyle/+}] (122) at (-0.75, 0.875) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (0.75, 0.875) {${a_1}$};
            \node [style=none] (124) at (-2, 1.875) {};
            \node [style=none] (125) at (-2, -1.875) {};
            \node [style=none] (126) at (2, -1.875) {};
            \node [style=none] (127) at (2, 1.875) {};
            \node [style=none] (131) at (-1.75, -0.125) {};
            \node [style=none] (132) at (-1.75, -1.625) {};
            \node [style=none] (133) at (1.75, -1.625) {};
            \node [style=none] (134) at (1.75, -0.125) {};
            \node [style=none] (135) at (1.75, -0.875) {};
            \node [{boxStyle/+}] (136) at (-0.75, -0.875) {$b_2$};
            \node [{boxOpStyle/-}] (137) at (0.75, -0.875) {${a_2}$};
            \node [style=none] (138) at (2, -0.875) {};
            \node [style=none] (139) at (2, 0.875) {};
            \node [style=none] (140) at (-2, -0.875) {};
            \node [style=none] (141) at (-2, 0.875) {};
            \node [style=none] (142) at (-1.75, -0.875) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [{bgStyle/-}] (133.center)
                 to (132.center)
                 to (131.center)
                 to (134.center)
                 to cycle;
            \draw [{wStyle/-}] (137) to (135.center);
            \draw [{wStyle/-}] (136) to (137);
            \draw [style={wStyle/+}] (138.center) to (135.center);
            \draw [style={wStyle/+}] (141.center) to (81.center);
            \draw [style={wStyle/+}] (121.center) to (139.center);
            \draw [style={wStyle/+}] (140.center) to (142.center);
            \draw [style={wStyle/-}] (142.center) to (136);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \stackrel{\eqref{ax:linStrn2}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (2.625, 0.875) {};
            \node [{boxOpStyle/-}] (122) at (1.75, 0.875) {${a_1}$};
            \node [{boxStyle/+}] (123) at (-0.125, 0.875) {$b_1$};
            \node [style=none] (124) at (2.875, 1.875) {};
            \node [style=none] (125) at (2.875, -1.875) {};
            \node [style=none] (126) at (-1.125, -1.875) {};
            \node [style=none] (127) at (-1.125, 1.875) {};
            \node [style=none] (131) at (2.625, 1.625) {};
            \node [style=none] (132) at (2.625, -1.625) {};
            \node [style=none] (133) at (0.875, -1.625) {};
            \node [style=none] (134) at (0.875, 1.625) {};
            \node [{boxOpStyle/-}] (136) at (1.75, -0.875) {${a_2}$};
            \node [{boxStyle/+}] (137) at (-0.125, -0.875) {$b_2$};
            \node [style=none] (138) at (-1.125, -0.875) {};
            \node [style=none] (139) at (-1.125, 0.875) {};
            \node [style=none] (140) at (2.875, -0.875) {};
            \node [style=none] (141) at (2.875, 0.875) {};
            \node [style=none] (142) at (2.625, -0.875) {};
            \node [style=none] (143) at (0.875, 0.875) {};
            \node [style=none] (144) at (0.875, -0.875) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (133.center)
                 to (132.center)
                 to (131.center)
                 to (134.center)
                 to cycle;
            \draw [style={wStyle/+}] (81.center) to (122);
            \draw [style={wStyle/+}] (122) to (143.center);
            \draw [style={wStyle/+}] (144.center) to (136);
            \draw [style={wStyle/+}] (136) to (142.center);
            \draw [style={wStyle/-}] (144.center) to (137);
            \draw [style={wStyle/-}] (137) to (138.center);
            \draw [style={wStyle/-}] (123) to (139.center);
            \draw [style={wStyle/-}] (123) to (143.center);
            \draw [style={wStyle/-}] (81.center) to (141.center);
            \draw [style={wStyle/-}] (140.center) to (142.center);
        \end{pgfonlayer}
    \end{tikzpicture}      
\]

==> tikz/proofs/deductionTheorem/tensorPlus.tex <==
\[
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, 0) {};
            \node [style=none] (112) at (-0.75, 1.25) {};
            \node [style=none] (113) at (-0.75, -1) {};
            \node [style=none] (114) at (0.75, -1) {};
            \node [style=none] (115) at (0.75, 1.25) {};
            \node [style=none] (121) at (0.75, 0) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (0, 0.65) {$c$};
            \node [style=none] (123) at (-0.75, -0.5) {};
            \node [style=none] (124) at (0.75, -0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
            \draw [{wStyle/+}] (123.center) to (124.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \stackrel{\eqref{ax:comPlusLaxNat}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, -0.675) {};
            \node [style=none] (112) at (-0.75, 1.575) {};
            \node [style=none] (113) at (-0.75, -1.675) {};
            \node [style=none] (114) at (0.75, -1.675) {};
            \node [style=none] (115) at (0.75, 1.575) {};
            \node [style=none] (121) at (0.75, -0.675) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (0, -0.025) {$c$};
            \node [style=none] (123) at (-0.75, -1.175) {};
            \node [style=none] (124) at (0.75, -1.175) {};
            \node [style={boxStyle/+}, scale=0.8] (125) at (0, 0.975) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
            \draw [{wStyle/+}] (123.center) to (124.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, 0.325) {};
            \node [style=none] (112) at (-0.75, 1.575) {};
            \node [style=none] (113) at (-0.75, -1.675) {};
            \node [style=none] (114) at (0.75, -1.675) {};
            \node [style=none] (115) at (0.75, 1.575) {};
            \node [style=none] (121) at (0.75, 0.325) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (0, -0.525) {$c$};
            \node [style=none] (123) at (-0.75, -1.175) {};
            \node [style=none] (124) at (0.75, -1.175) {};
            \node [style={boxStyle/+}, scale=0.8] (125) at (0, 0.975) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
            \draw [{wStyle/+}] (123.center) to (124.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \stackrel{\text{Ind. hyp.}}{\synequivalenceT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-1.75, 0.875) {};
            \node [style=none] (112) at (-1.75, 1.625) {};
            \node [style=none] (113) at (-1.75, 0.125) {};
            \node [style=none] (114) at (1.75, 0.125) {};
            \node [style=none] (115) at (1.75, 1.625) {};
            \node [style=none] (121) at (1.75, 0.875) {};
            \node [{boxStyle/+}] (122) at (-0.75, 0.875) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (0.75, 0.875) {${a_1}$};
            \node [style=none] (124) at (-2, 1.875) {};
            \node [style=none] (125) at (-2, -1.875) {};
            \node [style=none] (126) at (2, -1.875) {};
            \node [style=none] (127) at (2, 1.875) {};
            \node [style=none] (131) at (-1.75, -0.125) {};
            \node [style=none] (132) at (-1.75, -1.625) {};
            \node [style=none] (133) at (1.75, -1.625) {};
            \node [style=none] (134) at (1.75, -0.125) {};
            \node [style=none] (135) at (1.75, -0.875) {};
            \node [{boxStyle/+}] (136) at (-0.75, -0.875) {$b_2$};
            \node [{boxOpStyle/-}] (137) at (0.75, -0.875) {${a_2}$};
            \node [style=none] (138) at (2, -0.875) {};
            \node [style=none] (139) at (2, 0.875) {};
            \node [style=none] (140) at (-2, -0.875) {};
            \node [style=none] (141) at (-2, 0.875) {};
            \node [style=none] (142) at (-1.75, -0.875) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [{bgStyle/-}] (133.center)
                 to (132.center)
                 to (131.center)
                 to (134.center)
                 to cycle;
            \draw [{wStyle/-}] (137) to (135.center);
            \draw [{wStyle/-}] (136) to (137);
            \draw [style={wStyle/+}] (138.center) to (135.center);
            \draw [style={wStyle/+}] (141.center) to (81.center);
            \draw [style={wStyle/+}] (121.center) to (139.center);
            \draw [style={wStyle/+}] (140.center) to (142.center);
            \draw [style={wStyle/-}] (142.center) to (136);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \stackrel{\eqref{ax:linStrn1}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.875, 0.875) {};
            \node [{boxStyle/+}] (122) at (0, 0.875) {$b_1$};
            \node [{boxOpStyle/-}] (123) at (1.875, 0.875) {${a_1}$};
            \node [style=none] (124) at (-1.125, 1.875) {};
            \node [style=none] (125) at (-1.125, -1.875) {};
            \node [style=none] (126) at (2.875, -1.875) {};
            \node [style=none] (127) at (2.875, 1.875) {};
            \node [style=none] (131) at (-0.875, 1.625) {};
            \node [style=none] (132) at (-0.875, -1.625) {};
            \node [style=none] (133) at (0.875, -1.625) {};
            \node [style=none] (134) at (0.875, 1.625) {};
            \node [{boxStyle/+}] (136) at (0, -0.875) {$b_2$};
            \node [{boxOpStyle/-}] (137) at (1.875, -0.875) {${a_2}$};
            \node [style=none] (138) at (2.875, -0.875) {};
            \node [style=none] (139) at (2.875, 0.875) {};
            \node [style=none] (140) at (-1.125, -0.875) {};
            \node [style=none] (141) at (-1.125, 0.875) {};
            \node [style=none] (142) at (-0.875, -0.875) {};
            \node [style=none] (143) at (0.875, 0.875) {};
            \node [style=none] (144) at (0.875, -0.875) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (133.center)
                 to (132.center)
                 to (131.center)
                 to (134.center)
                 to cycle;
            \draw [style={wStyle/+}] (81.center) to (122);
            \draw [style={wStyle/+}] (122) to (143.center);
            \draw [style={wStyle/+}] (144.center) to (136);
            \draw [style={wStyle/+}] (136) to (142.center);
            \draw [style={wStyle/-}] (144.center) to (137);
            \draw [style={wStyle/-}] (137) to (138.center);
            \draw [style={wStyle/-}] (123) to (139.center);
            \draw [style={wStyle/-}] (123) to (143.center);
            \draw [style={wStyle/-}] (81.center) to (141.center);
            \draw [style={wStyle/-}] (140.center) to (142.center);
        \end{pgfonlayer}
    \end{tikzpicture}     
\]

==> tikz/proofs/deductionTheorem/transitivity.tex <==
\[
\begin{array}{rcl}
    \tikzfig{cPerId} 
    &\stackrel{\eqref{ax:comPlusLaxNat}}{\syninclusionT{\T{T}}}&
    \tikzfig{cPerCperId} 
    \structuralcong
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-0.75, 0) {};
            \node [style=none] (112) at (-0.75, 1.25) {};
            \node [style=none] (113) at (-0.75, -0.75) {};
            \node [style=none] (114) at (2, -0.75) {};
            \node [style=none] (115) at (2, 1.25) {};
            \node [style=none] (121) at (2, 0) {};
            \node [style={boxStyle/+}, scale=0.8] (122) at (1.25, 0.65) {$c$};
            \node [style={boxStyle/+}, scale=0.8] (123) at (0, 0.65) {$c$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/+}] (81.center) to (121.center);
        \end{pgfonlayer}
    \end{tikzpicture}    
    \stackrel{\text{Ind. hyp.}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, 0) {};
            \node [style=none] (112) at (-3.75, 0.75) {};
            \node [style=none] (113) at (-3.75, -0.75) {};
            \node [style=none] (114) at (-0.25, -0.75) {};
            \node [style=none] (115) at (-0.25, 0.75) {};
            \node [style=none] (121) at (-0.25, 0) {};
            \node [{boxStyle/+}] (122) at (-2.75, 0) {$b$};
            \node [{boxOpStyle/-}] (123) at (-1.25, 0) {$d$};
            \node [style=none] (124) at (-4, 1) {};
            \node [style=none] (125) at (-4, -1) {};
            \node [style=none] (126) at (3.75, -1) {};
            \node [style=none] (127) at (3.75, 1) {};
            \node [style=none] (128) at (-4, 0) {};
            \node [style=none] (130) at (0, 0) {};
            \node [style=none] (131) at (0, 0.75) {};
            \node [style=none] (132) at (0, -0.75) {};
            \node [style=none] (133) at (3.5, -0.75) {};
            \node [style=none] (134) at (3.5, 0.75) {};
            \node [style=none] (135) at (3.5, 0) {};
            \node [{boxStyle/+}] (136) at (1, 0) {$d$};
            \node [{boxOpStyle/-}] (137) at (2.5, 0) {$a$};
            \node [style=none] (138) at (3.75, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [style={wStyle/+}] (81.center) to (128.center);
            \draw [{bgStyle/-}] (133.center)
                 to (132.center)
                 to (131.center)
                 to (134.center)
                 to cycle;
            \draw [{wStyle/-}] (130.center) to (136);
            \draw [{wStyle/-}] (137) to (135.center);
            \draw [{wStyle/-}] (136) to (137);
            \draw [style={wStyle/+}] (130.center) to (121.center);
            \draw [style={wStyle/+}] (138.center) to (135.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \stackrel{\eqref{ax:leftLinDistr}}{\syninclusionT{\T{T}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (-3.75, 0) {};
            \node [style=none] (112) at (-3.75, 0.75) {};
            \node [style=none] (113) at (-3.75, -0.75) {};
            \node [style=none] (114) at (-0.25, -0.75) {};
            \node [style=none] (115) at (-0.25, 0.75) {};
            \node [style=none] (121) at (-0.25, 0) {};
            \node [{boxStyle/+}] (122) at (-2.75, 0) {$b$};
            \node [{boxOpStyle/-}] (123) at (-1.25, 0) {$d$};
            \node [style=none] (124) at (-4, 1) {};
            \node [style=none] (125) at (-4, -1) {};
            \node [style=none] (126) at (1.25, -1) {};
            \node [style=none] (127) at (1.25, 1) {};
            \node [style=none] (128) at (-4, 0) {};
            \node [style=none] (135) at (1.25, 0) {};
            \node [{boxStyle/+}] (136) at (0.5, 0) {$d$};
            \node [{boxOpStyle/-}] (137) at (2.25, 0) {$a$};
            \node [style=none] (138) at (-4.25, 1.25) {};
            \node [style=none] (139) at (-4.25, -1.25) {};
            \node [style=none] (140) at (3.25, -1.25) {};
            \node [style=none] (141) at (3.25, 1.25) {};
            \node [style=none] (142) at (3.25, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (140.center)
                 to (139.center)
                 to (138.center)
                 to (141.center)
                 to cycle;
            \draw [{bgStyle/+}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/-}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [{wStyle/-}] (81.center) to (122);
            \draw [{wStyle/-}] (123) to (121.center);
            \draw [{wStyle/-}] (122) to (123);
            \draw [style={wStyle/+}] (81.center) to (128.center);
            \draw [style={wStyle/+}] (121.center) to (136);
            \draw [style={wStyle/+}] (136) to (135.center);
            \draw [style={wStyle/-}] (135.center) to (137);
            \draw [style={wStyle/-}] (137) to (142.center);
        \end{pgfonlayer}
    \end{tikzpicture} \\[15pt]
    &\stackrel{\eqref{ax:rightLinDistr}}{\syninclusionT{\T{T}}}&
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (81) at (1.575, 0) {};
            \node [style=none] (112) at (1.575, 0.75) {};
            \node [style=none] (113) at (1.575, -0.75) {};
            \node [style=none] (114) at (-1.75, -0.75) {};
            \node [style=none] (115) at (-1.75, 0.75) {};
            \node [style=none] (121) at (-1.75, 0) {};
            \node [{boxStyle/+}] (122) at (0.75, 0) {$d$};
            \node [{boxOpStyle/-}] (123) at (-0.75, 0) {$d$};
            \node [style=none] (124) at (3.25, 1) {};
            \node [style=none] (125) at (3.25, -1) {};
            \node [style=none] (126) at (-3.25, -1) {};
            \node [style=none] (127) at (-3.25, 1) {};
            \node [style=none] (135) at (-3.25, 0) {};
            \node [{boxStyle/+}] (136) at (-2.5, 0) {$b$};
            \node [{boxOpStyle/-}] (137) at (2.5, 0) {$a$};
            \node [style=none] (142) at (3.25, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (126.center)
                 to (125.center)
                 to (124.center)
                 to (127.center)
                 to cycle;
            \draw [{bgStyle/+}] (114.center)
                 to (113.center)
                 to (112.center)
                 to (115.center)
                 to cycle;
            \draw [style={wStyle/-}] (137) to (142.center);
            \draw [style={wStyle/+}] (121.center) to (123);
            \draw [style={wStyle/+}] (123) to (122);
            \draw [style={wStyle/+}] (122) to (81.center);
            \draw [style={wStyle/-}] (135.center) to (136);
            \draw [style={wStyle/-}] (136) to (121.center);
            \draw [style={wStyle/-}] (81.center) to (137);
        \end{pgfonlayer}
    \end{tikzpicture}       
    \stackrel{\rla{d} \Vdash d}{\syninclusionT{\T{T}}}\!\!\!\!
    \seqCirc[-]{b}{a}[][][w][b]
\end{array}
\]

==> tikz/proofs/henkinProp/seqPlus.tex <==
\[
    \allowdisplaybreaks
    \begin{array}{r@{}c@{}l}
        \HenFunctor(\scalebox{0.8}{\seqCirc[+]{c}{d}}) &\Leq{\text{Def. }\HenFunctor}&  \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \seq[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \\[8pt]
                                                &\Leq{\text{Ind. hyp.}}&                     \{ (\nterm{k},\nterm{t}) \in X^n\times X^o \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \} \seq[+] \{ (\nterm{t},\nterm{l}) \in X^o\times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[8pt]
                                                &\Leq{\eqref{eq:seqRel}}&                                          \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \wedge \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[-5pt]
                                                &\Leq{\footnotesize{\stackanchor{\eqref{ax:comPlusLaxNat}}{\eqref{ax:discPlusLaxNat}}}}&                 \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinTensor}} \} \\[10pt]
                                                &\structuralcong&                           \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinSeq}} \} \\[8pt]
                                                &\stackrel{\text{Prop. }~\ref{prop:map adj}}{\subseteq}&                \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinSeq2}} \}
    \end{array}
\]

% \[
%     \begin{array}{rcl}
%         \HenFunctor(\scalebox{0.8}{\seqCirc[+]{c}{d}}) &\Leq{\text{Def. }\ref{def:henkin struct}}&  \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \seq[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \\[8pt]
%                                                 &\Leq{\text{Ind. hyp.}}&                     \{ (t,t'') \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{t}{c}{t''}} \} \seq[+] \{ (t'',t') \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{t''}{d}{t'}} \} \\[8pt]
%                                                 &=&                                          \{ (t,t') \mid \exists t'' \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{t}{c}{t''}} \wedge \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{t''}{d}{t'}} \} \\[8pt]
%                                                 &\Leq{\text{Lemma }~\ref{}}&                 \{ (t,t') \mid \exists t'' \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinTensor}} \} \\[10pt]
%                                                 &\Leq{\text{SMC}}&                           \{ (t,t') \mid \exists t'' \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinSeq}} \} \\[8pt]
%                                                 % &\Leq{\text{Lemma }~\ref{}}&                \{ (t,t') \mid \exists t'' \; \scalebox{0.8}{\emptyCirc[+]} \leq \scalebox{0.8}{\tikzfig{henkinSeq}} \leq \scalebox{0.8}{\tikzfig{henkinSeq2}} \} \\[8pt]
%                                                 &\stackrel{\text{Lemma }~\ref{}}{\subseteq}& \{ (t,t') \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinSeq2}} \}
%                                                 % &=&                                          \{ (t,t') \mid \scalebox{0.8}{\emptyCirc[+]} \leq \scalebox{0.8}{\tikzfig{henkinSeq2}} \}
%     \end{array}
% \]

For the other inclusion the following holds:

\[
    \allowdisplaybreaks
    \begin{array}{r@{}c@{}l}
        & & \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinSeq2}} \} \stackrel{\eqref{eqdagger}}{=} \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \scalebox{0.8}{\emptyCirc[+]}
        \precongR{\T{T}}
        \;\scalebox{0.8}{\begin{tikzpicture}
            \begin{pgfonlayer}{nodelayer}
                \node [style=none] (122) at (2.75, 1.35) {};
                \node [style=none] (123) at (2.75, -1.4) {};
                \node [style=none] (124) at (-2.2, -1.4) {};
                \node [style=none] (125) at (-2.2, 1.35) {};
                \node [{boxStyle/+}] (127) at (0.675, -0.65) {$d$};
                \node [{funcOpStyle/+}] (133) at (1.95, -0.65) {$\nterm{l}$};
                \node [{boxOpStyle/+}] (134) at (0.675, 0.6) {$c$};
                \node [{funcOpStyle/+}] (135) at (1.95, 0.6) {$\nterm{k}$};
                \node [style={dotStyle/+}] (136) at (-0.25, 0) {};
                \node [style={dotStyle/+}] (137) at (-1.25, 0) {};
            \end{pgfonlayer}
            \begin{pgfonlayer}{edgelayer}
                \draw [{bgStyle/+}] (124.center)
                     to (123.center)
                     to (122.center)
                     to (125.center)
                     to cycle;
                \draw [style={wStyle/+}] (127) to (133);
                \draw [style={wStyle/+}] (134) to (135);
                \draw [style={wStyle/+}] (136) to (137);
                \draw [style={wStyle/+}, bend left] (136) to (134);
                \draw [style={wStyle/+}, bend right] (136) to (127);
            \end{pgfonlayer}
        \end{tikzpicture}    
        } \} \\
        &\stackrel{\text{Lemma }\ref{lemma:henkinn}}{\subseteq}& \{ (\nterm{k},\nterm{l}) \in X^n \times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]}
        \precongR{\T{T}} \scalebox{0.8}{\begin{tikzpicture}
            \begin{pgfonlayer}{nodelayer}
                \node [style=none] (122) at (2.75, 1.35) {};
                \node [style=none] (123) at (2.75, -1.4) {};
                \node [style=none] (124) at (-2.2, -1.4) {};
                \node [style=none] (125) at (-2.2, 1.35) {};
                \node [{boxStyle/+}] (127) at (0.675, -0.65) {$d$};
                \node [{funcOpStyle/+}] (133) at (1.95, -0.65) {$\nterm{l}$};
                \node [{boxOpStyle/+}] (134) at (0.675, 0.6) {$c$};
                \node [{funcOpStyle/+}] (135) at (1.95, 0.6) {$\nterm{k}$};
                \node [style={dotStyle/+}] (136) at (-0.25, 0) {};
                \node [style={funcStyle/+}] (137) at (-1.25, 0) {$\nterm{t}$};
            \end{pgfonlayer}
            \begin{pgfonlayer}{edgelayer}
                \draw [{bgStyle/+}] (124.center)
                     to (123.center)
                     to (122.center)
                     to (125.center)
                     to cycle;
                \draw [style={wStyle/+}] (127) to (133);
                \draw [style={wStyle/+}] (134) to (135);
                \draw [style={wStyle/+}] (136) to (137);
                \draw [style={wStyle/+}, bend left] (136) to (134);
                \draw [style={wStyle/+}, bend right] (136) to (127);
            \end{pgfonlayer}
        \end{tikzpicture}    
        } \} \stackrel{\eqref{TMAPk}}{=} \{ (\nterm{k},\nterm{l}) \in X^n \times X^m \mid  \exists \nterm{t} \;  \scalebox{0.8}{\emptyCirc[+]}
        \precongR{\T{T}} \scalebox{0.8}{
            \begin{tikzpicture}
                \begin{pgfonlayer}{nodelayer}
                    \node [{boxOpStyle/+}] (107) at (-0.025, 0.65) {$c$};
                    \node [{funcStyle/+}] (117) at (-1.25, 0.65) {$\nterm{t}$};
                    \node [style=none] (122) at (2, 1.4) {};
                    \node [style=none] (123) at (2, -1.4) {};
                    \node [style=none] (124) at (-1.95, -1.4) {};
                    \node [style=none] (125) at (-1.95, 1.4) {};
                    \node [{funcOpStyle/+}] (126) at (1.25, 0.65) {$\nterm{k}$};
                    \node [{boxStyle/+}] (127) at (0, -0.65) {$d$};
                    \node [{funcStyle/+}] (128) at (-1.225, -0.65) {$\nterm{t}$};
                    \node [{funcOpStyle/+}] (133) at (1.275, -0.65) {$\nterm{l}$};
                \end{pgfonlayer}
                \begin{pgfonlayer}{edgelayer}
                    \draw [{bgStyle/+}] (124.center)
                         to (123.center)
                         to (122.center)
                         to (125.center)
                         to cycle;
                    \draw [style={wStyle/+}] (107) to (126);
                    \draw [style={wStyle/+}] (117) to (107);
                    \draw [style={wStyle/+}] (127) to (133);
                    \draw [style={wStyle/+}] (128) to (127);
                \end{pgfonlayer}
            \end{tikzpicture}                    
        } \} \\[-8pt]
        &\Leq{\footnotesize{\stackanchor{\eqref{ax:comPlusLaxNat}}{\eqref{ax:discPlusLaxNat}}}}&  \{ (\nterm{k},\nterm{l}) \in X^n \times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedOpFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \wedge \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[3pt]
        &\Leq{\eqref{eq:seqRel}}&                          \{ (\nterm{k},\nterm{t}) \in X^n \times X^o \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedOpFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \} \seq[+] \{ (\nterm{t},\nterm{l}) \in X^o \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[3pt]
        &\stackrel{\text{Table }\ref{table:daggerproperties}}{=}&                          \{ (\nterm{k},\nterm{t}) \in X^n \times X^o \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \} \seq[+] \{ (\nterm{t},\nterm{l}) \in X^o \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[3pt]
        &\Leq{\text{Ind. hyp.}}&     \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \seq[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \Leq{\text{Def. }\HenFunctor} \HenFunctor(\scalebox{0.8}{\seqCirc[+]{c}{d}})
    \end{array}
\]


    % {\allowdisplaybreaks
    % \begin{align*}
    %     & \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\tikzfig{henkinSeq2}} \}\\[8pt]
    %      &\stackrel{\eqref{eqdagger}}{=} \{ (\nterm{k},\nterm{l}) \in X^n\times X^m \mid \scalebox{0.8}{\emptyCirc[+]}
    %     \precongR{\T{T}}
    %     \;\scalebox{0.8}{\begin{tikzpicture}
    %         \begin{pgfonlayer}{nodelayer}
    %             \node [style=none] (122) at (2.75, 1.35) {};
    %             \node [style=none] (123) at (2.75, -1.4) {};
    %             \node [style=none] (124) at (-2.2, -1.4) {};
    %             \node [style=none] (125) at (-2.2, 1.35) {};
    %             \node [{boxStyle/+}] (127) at (0.675, -0.65) {$d$};
    %             \node [{funcOpStyle/+}] (133) at (1.95, -0.65) {$\nterm{l}$};
    %             \node [{boxOpStyle/+}] (134) at (0.675, 0.6) {$c$};
    %             \node [{funcOpStyle/+}] (135) at (1.95, 0.6) {$\nterm{k}$};
    %             \node [style={dotStyle/+}] (136) at (-0.25, 0) {};
    %             \node [style={dotStyle/+}] (137) at (-1.25, 0) {};
    %         \end{pgfonlayer}
    %         \begin{pgfonlayer}{edgelayer}
    %             \draw [{bgStyle/+}] (124.center)
    %                  to (123.center)
    %                  to (122.center)
    %                  to (125.center)
    %                  to cycle;
    %             \draw [style={wStyle/+}] (127) to (133);
    %             \draw [style={wStyle/+}] (134) to (135);
    %             \draw [style={wStyle/+}] (136) to (137);
    %             \draw [style={wStyle/+}, bend left] (136) to (134);
    %             \draw [style={wStyle/+}, bend right] (136) to (127);
    %         \end{pgfonlayer}
    %     \end{tikzpicture}    
    %     } \} \\[12pt]
    %     &\stackrel{\text{Lemma }\ref{lemma:henkinn}}{\subseteq} \{ (\nterm{k},\nterm{l}) \in X^n \times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]}
    %     \precongR{\T{T}} \scalebox{0.8}{\begin{tikzpicture}
    %         \begin{pgfonlayer}{nodelayer}
    %             \node [style=none] (122) at (2.75, 1.35) {};
    %             \node [style=none] (123) at (2.75, -1.4) {};
    %             \node [style=none] (124) at (-2.2, -1.4) {};
    %             \node [style=none] (125) at (-2.2, 1.35) {};
    %             \node [{boxStyle/+}] (127) at (0.675, -0.65) {$d$};
    %             \node [{funcOpStyle/+}] (133) at (1.95, -0.65) {$\nterm{l}$};
    %             \node [{boxOpStyle/+}] (134) at (0.675, 0.6) {$c$};
    %             \node [{funcOpStyle/+}] (135) at (1.95, 0.6) {$\nterm{k}$};
    %             \node [style={dotStyle/+}] (136) at (-0.25, 0) {};
    %             \node [style={funcStyle/+}] (137) at (-1.25, 0) {$\nterm{t}$};
    %         \end{pgfonlayer}
    %         \begin{pgfonlayer}{edgelayer}
    %             \draw [{bgStyle/+}] (124.center)
    %                  to (123.center)
    %                  to (122.center)
    %                  to (125.center)
    %                  to cycle;
    %             \draw [style={wStyle/+}] (127) to (133);
    %             \draw [style={wStyle/+}] (134) to (135);
    %             \draw [style={wStyle/+}] (136) to (137);
    %             \draw [style={wStyle/+}, bend left] (136) to (134);
    %             \draw [style={wStyle/+}, bend right] (136) to (127);
    %         \end{pgfonlayer}
    %     \end{tikzpicture}    
    %     } \} \\[12pt]
    %     &\stackrel{\eqref{TMAPk}}{=} \{ (\nterm{k},\nterm{l}) \in X^n \times X^m \mid  \exists \nterm{t} \;  \scalebox{0.8}{\emptyCirc[+]}
    %     \precongR{\T{T}} \scalebox{0.8}{
    %         \begin{tikzpicture}
    %             \begin{pgfonlayer}{nodelayer}
    %                 \node [{boxOpStyle/+}] (107) at (-0.025, 0.65) {$c$};
    %                 \node [{funcStyle/+}] (117) at (-1.25, 0.65) {$\nterm{t}$};
    %                 \node [style=none] (122) at (2, 1.4) {};
    %                 \node [style=none] (123) at (2, -1.4) {};
    %                 \node [style=none] (124) at (-1.95, -1.4) {};
    %                 \node [style=none] (125) at (-1.95, 1.4) {};
    %                 \node [{funcOpStyle/+}] (126) at (1.25, 0.65) {$\nterm{k}$};
    %                 \node [{boxStyle/+}] (127) at (0, -0.65) {$d$};
    %                 \node [{funcStyle/+}] (128) at (-1.225, -0.65) {$\nterm{t}$};
    %                 \node [{funcOpStyle/+}] (133) at (1.275, -0.65) {$\nterm{l}$};
    %             \end{pgfonlayer}
    %             \begin{pgfonlayer}{edgelayer}
    %                 \draw [{bgStyle/+}] (124.center)
    %                      to (123.center)
    %                      to (122.center)
    %                      to (125.center)
    %                      to cycle;
    %                 \draw [style={wStyle/+}] (107) to (126);
    %                 \draw [style={wStyle/+}] (117) to (107);
    %                 \draw [style={wStyle/+}] (127) to (133);
    %                 \draw [style={wStyle/+}] (128) to (127);
    %             \end{pgfonlayer}
    %         \end{tikzpicture}                    
    %     } \} \\
    %     &\Leq{\footnotesize{\stackanchor{\eqref{ax:comPlusLaxNat}}{\eqref{ax:discPlusLaxNat}}}}  \{ (\nterm{k},\nterm{l}) \in X^n \times X^m \mid \exists \nterm{t} \; \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedOpFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \wedge \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[8pt]
    %     &\Leq{\eqref{eq:seqRel}}                          \{ (\nterm{k},\nterm{t}) \in X^n \times X^o \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedOpFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \} \seq[+] \{ (\nterm{t},\nterm{l}) \in X^o \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[3pt]
    %     &\stackrel{\text{Table }\ref{table:daggerproperties}}{=}                          \{ (\nterm{k},\nterm{t}) \in X^n \times X^o \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k}}{c}{\nterm{t}}} \} \seq[+] \{ (\nterm{t},\nterm{l}) \in X^o \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{t}}{d}{\nterm{l}}} \} \\[3pt]
    %     &\Leq{\text{Ind. hyp.}}     \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \seq[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \\
    %     &\Leq{\text{Def. }\HenFunctor} \HenFunctor(\scalebox{0.8}{\seqCirc[+]{c}{d}})
    % \end{align*}}

==> tikz/proofs/henkinProp/tensorPlus.tex <==

{\allowdisplaybreaks
    \begin{align*}
        \HenFunctor(\scalebox{0.8}{\tensorCirc[+]{c}{d}}) \Leq{\text{Def. }\HenFunctor}&  \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \tensor[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \\[8pt]
                                                   \Leq{\text{Ind. hyp.}}&                      \{ (\nterm{k_1},\nterm{l_1} \in X^n \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_1}}{c}{\nterm{l_1}}} \} \tensor[+] \{ (\nterm{k_2},\nterm{l_2}) \in X^o \times X^p \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_2}}{d}{\nterm{l_2}}} \} \\[8pt]
                                                   \Leq{\eqref{eq:tensorREL}} \;\;\;&                                           \{ ( \Bigl( \begin{smallmatrix} \nterm{k_1} \\ \nterm{k_2} \end{smallmatrix} \Bigr), \Bigl( \begin{smallmatrix} \nterm{l_1} \\ \nterm{l_2} \end{smallmatrix} \Bigr) ) \in X^{n+o} \times X^{m+p} \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_1}}{c}{\nterm{l_1}}} \wedge \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_2}}{d}{\nterm{l_2}}} \} \\[-5pt]
                                                   \Leq{\footnotesize{\stackanchor{\eqref{ax:comPlusLaxNat}}{\eqref{ax:discPlusLaxNat}}}}\;\;\;&                  \{ ( \Bigl( \begin{smallmatrix} \nterm{k_1} \\ \nterm{k_2} \end{smallmatrix} \Bigr), \Bigl( \begin{smallmatrix} \nterm{l_1} \\ \nterm{l_2} \end{smallmatrix} \Bigr) ) \in X^{n+o} \times X^{m+p} \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{{T}}} \scalebox{0.8}{\closedDecomposedTensorCirc{\nterm{k_1}}{\nterm{k_2}}{c}{d}{\nterm{l_1}}{\nterm{l_2}}} \} \\[3pt]
                                                   \Leq{\text{Prop. }~\ref{prop:nary maps}}&                                           \{ (\nterm{k}, \nterm{l}) \in X^{n+o} \times X^{m+p} \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedTensorCirc{k}{c}{d}{l}} \, , \nterm{k} = \nterm{k_1} \tensor[+] \nterm{k_2}, \nterm{l} = \nterm{l_1} \tensor[+] \nterm{l_2} \}
    \end{align*}
}

==> tikz/proofs/implication/capped.tex <==

\[
    \cappedCirc[+]{b}
    \Lleq{\text{Lemma }~\ref{lm:id cup}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (109) at (-1.25, 0.25) {};
            \node [style=none] (122) at (-1.25, -1.125) {};
            \node [style=none] (123) at (-1.25, 1.05) {};
            \node [style=none] (124) at (3.375, 1.05) {};
            \node [style=none] (125) at (3.375, -1.125) {};
            \node [{dotStyle/-}] (128) at (2.125, -0.125) {};
            \node [style=none] (129) at (1.625, 0.25) {};
            \node [style=none] (130) at (1.625, -0.5) {};
            \node [{dotStyle/-}] (131) at (2.75, -0.125) {};
            \node [style=none] (133) at (-1.25, -0.5) {};
            \node [{boxStyle/+}] (134) at (-0.5, 0.25) {$b$};
            \node [style=none] (135) at (0.25, -0.875) {};
            \node [style=none] (136) at (0.25, 0.8) {};
            \node [style=none] (137) at (3.125, 0.8) {};
            \node [style=none] (138) at (3.125, -0.875) {};
            \node [style=none] (139) at (0.25, 0.25) {};
            \node [style=none] (140) at (0.625, 0.25) {};
            \node [style=none] (141) at (0.625, 0) {};
            \node [style=none] (142) at (0.625, 0.5) {};
            \node [style=none] (143) at (1.625, 0.5) {};
            \node [style=none] (144) at (1.625, 0) {};
            \node [style=none] (145) at (0.25, -0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{bgStyle/-}] (137.center)
                 to (136.center)
                 to (135.center)
                 to (138.center)
                 to cycle;
            \draw [{bgStyle/+}] (144.center)
                 to (143.center)
                 to (142.center)
                 to (141.center)
                 to cycle;
            \draw [{wStyle/-}, bend right] (130.center) to (128);
            \draw [{wStyle/-}, bend right] (128) to (129.center);
            \draw [{wStyle/-}] (128) to (131);
            \draw [{wStyle/+}] (109.center) to (134);
            \draw [style={wStyle/+}] (134) to (139.center);
            \draw [style={wStyle/-}] (139.center) to (140.center);
            \draw [style={wStyle/+}] (140.center) to (129.center);
            \draw [style={wStyle/+}] (145.center) to (133.center);
            \draw [style={wStyle/-}] (130.center) to (145.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \Lleq{\eqref{ax:leftLinDistr}} 
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (109) at (-1, 0.25) {};
            \node [style=none] (122) at (-1.25, -1.125) {};
            \node [style=none] (123) at (-1.25, 1.1) {};
            \node [style=none] (124) at (3.625, 1.1) {};
            \node [style=none] (125) at (3.625, -1.125) {};
            \node [{dotStyle/-}] (128) at (2.625, -0.125) {};
            \node [style=none] (129) at (2.125, 0.25) {};
            \node [style=none] (130) at (2.125, -0.5) {};
            \node [{dotStyle/-}] (131) at (3.25, -0.125) {};
            \node [style=none] (133) at (-1, -0.5) {};
            \node [{boxStyle/+}] (134) at (-0.25, 0.25) {$b$};
            \node [style=none] (135) at (-1, -0.875) {};
            \node [style=none] (136) at (-1, 0.85) {};
            \node [style=none] (137) at (2.125, 0.85) {};
            \node [style=none] (138) at (2.125, -0.875) {};
            \node [style=none] (139) at (0.5, 0.25) {};
            \node [style=none] (141) at (0.7, 0) {};
            \node [style=none] (142) at (0.7, 0.5) {};
            \node [style=none] (143) at (1.7, 0.5) {};
            \node [style=none] (144) at (1.7, 0) {};
            \node [style=none] (145) at (0.5, -0.5) {};
            \node [style=none] (146) at (0.5, -0.75) {};
            \node [style=none] (147) at (0.5, 0.725) {};
            \node [style=none] (148) at (1.875, 0.725) {};
            \node [style=none] (149) at (1.875, -0.75) {};
            \node [style=none] (150) at (1.875, 0.25) {};
            \node [style=none] (151) at (1.875, -0.5) {};
            \node [style=none] (152) at (1.7, 0.25) {};
            \node [style=none] (153) at (0.7, 0.25) {};
            \node [style=none] (154) at (-1.25, 0.25) {};
            \node [style=none] (155) at (-1.25, -0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{bgStyle/+}] (137.center)
                 to (136.center)
                 to (135.center)
                 to (138.center)
                 to cycle;
            \draw [{bgStyle/-}] (149.center)
                 to (148.center)
                 to (147.center)
                 to (146.center)
                 to cycle;
            \draw [{bgStyle/+}] (144.center)
                 to (143.center)
                 to (142.center)
                 to (141.center)
                 to cycle;
            \draw [{wStyle/-}, bend right] (130.center) to (128);
            \draw [{wStyle/-}, bend right] (128) to (129.center);
            \draw [{wStyle/+}] (109.center) to (134);
            \draw [style={wStyle/+}] (134) to (139.center);
            \draw [style={wStyle/+}] (145.center) to (133.center);
            \draw [style={wStyle/-}] (139.center) to (153.center);
            \draw [style={wStyle/-}] (152.center) to (150.center);
            \draw [style={wStyle/+}] (129.center) to (150.center);
            \draw [style={wStyle/+}] (153.center) to (152.center);
            \draw [style={wStyle/-}] (151.center) to (145.center);
            \draw [style={wStyle/-}] (154.center) to (109.center);
            \draw [style={wStyle/-}] (155.center) to (133.center);
            \draw [style={wStyle/-}] (128) to (131);
            \draw [style={wStyle/+}] (151.center) to (130.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \Lleq{\eqref{ax:linStrn4}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (109) at (-0.9, 0.5) {};
            \node [style=none] (122) at (-1.25, -1.25) {};
            \node [style=none] (123) at (-1.25, 1.35) {};
            \node [style=none] (124) at (3.15, 1.35) {};
            \node [style=none] (125) at (3.15, -1.25) {};
            \node [{dotStyle/-}] (128) at (2.15, -0.075) {};
            \node [style=none] (129) at (1.475, 0.5) {};
            \node [style=none] (130) at (1.475, -0.625) {};
            \node [{dotStyle/-}] (131) at (2.775, -0.075) {};
            \node [style=none] (133) at (-0.9, -0.625) {};
            \node [{boxStyle/+}] (134) at (-0.25, 0.5) {$b$};
            \node [style=none] (141) at (-0.9, -0.1) {};
            \node [style=none] (142) at (-0.9, 1.1) {};
            \node [style=none] (143) at (1.2, 1.1) {};
            \node [style=none] (144) at (1.2, -0.1) {};
            \node [style=none] (151) at (1.2, -0.625) {};
            \node [style=none] (152) at (1.2, 0.5) {};
            \node [style=none] (154) at (-1.25, 0.5) {};
            \node [style=none] (155) at (-1.25, -0.625) {};
            \node [style=none] (156) at (-0.9, -1) {};
            \node [style=none] (157) at (-0.9, -0.275) {};
            \node [style=none] (158) at (1.2, -0.275) {};
            \node [style=none] (159) at (1.2, -1) {};
            \node [style=none] (160) at (0.15, -0.85) {};
            \node [style=none] (161) at (0.15, -0.425) {};
            \node [style=none] (162) at (1, -0.425) {};
            \node [style=none] (163) at (1, -0.85) {};
            \node [style=none] (164) at (0.15, -0.625) {};
            \node [style=none] (165) at (1, -0.625) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{bgStyle/+}] (144.center)
                 to (143.center)
                 to (142.center)
                 to (141.center)
                 to cycle;
            \draw [{bgStyle/+}] (159.center)
                 to (158.center)
                 to (157.center)
                 to (156.center)
                 to cycle;
            \draw [{bgStyle/-}] (163.center)
                 to (162.center)
                 to (161.center)
                 to (160.center)
                 to cycle;
            \draw [{wStyle/-}, bend right] (130.center) to (128);
            \draw [{wStyle/-}, bend right] (128) to (129.center);
            \draw [style={wStyle/-}] (154.center) to (109.center);
            \draw [style={wStyle/-}] (155.center) to (133.center);
            \draw [style={wStyle/-}] (128) to (131);
            \draw [style={wStyle/+}] (109.center) to (134);
            \draw [style={wStyle/+}] (134) to (152.center);
            \draw [style={wStyle/-}] (152.center) to (129.center);
            \draw [style={wStyle/-}] (151.center) to (130.center);
            \draw [style={wStyle/-}] (164.center) to (165.center);
            \draw [style={wStyle/+}] (165.center) to (151.center);
            \draw [style={wStyle/+}] (164.center) to (133.center);
        \end{pgfonlayer}
    \end{tikzpicture}                                           
    \structuralcong
    \cappedCirc[-]{b}
\]
% \[
%     \circleCirc{\rla{b}}{b}
%     \Lgeq{b \Vdash \rla{b}}
%     \begin{tikzpicture}
%         \begin{pgfonlayer}{nodelayer}
%             \node [style=none] (122) at (2.125, -1) {};
%             \node [style=none] (123) at (2.125, 1) {};
%             \node [style=none] (124) at (-2.125, 1) {};
%             \node [style=none] (125) at (-2.125, -1) {};
%             \node [{dotStyle/-}] (128) at (-1.125, -0.125) {};
%             \node [style=none] (129) at (-0.5, 0.375) {};
%             \node [style=none] (130) at (-0.5, -0.625) {};
%             \node [{dotStyle/-}] (131) at (-1.75, -0.125) {};
%             \node [style=none] (133) at (0, -0.625) {};
%             \node [{dotStyle/-}] (135) at (1.125, -0.125) {};
%             \node [style=none] (136) at (0.5, 0.375) {};
%             \node [style=none] (137) at (0.5, -0.625) {};
%             \node [{dotStyle/-}] (138) at (1.75, -0.125) {};
%             \node [style=none] (139) at (0.5, 0.1) {};
%             \node [style=none] (140) at (0.5, 0.675) {};
%             \node [style=none] (141) at (-0.5, 0.675) {};
%             \node [style=none] (142) at (-0.5, 0.1) {};
%         \end{pgfonlayer}
%         \begin{pgfonlayer}{edgelayer}
%             \draw [{bgStyle/-}] (124.center)
%                  to (123.center)
%                  to (122.center)
%                  to (125.center)
%                  to cycle;
%             \draw [{bgStyle/+}] (141.center)
%                  to (140.center)
%                  to (139.center)
%                  to (142.center)
%                  to cycle;
%             \draw [{wStyle/-}, bend left] (130.center) to (128);
%             \draw [{wStyle/-}, bend left] (128) to (129.center);
%             \draw [{wStyle/-}] (128) to (131);
%             \draw [{wStyle/-}] (130.center) to (133.center);
%             \draw [{wStyle/-}, bend right] (137.center) to (135);
%             \draw [{wStyle/-}, bend right] (135) to (136.center);
%             \draw [{wStyle/-}] (135) to (138);
%             \draw [style={wStyle/-}] (133.center) to (137.center);
%             \draw [style={wStyle/+}] (129.center) to (136.center);
%         \end{pgfonlayer}
%     \end{tikzpicture}
%     \Lgeq{\text{Lemma }~\ref{lm:bool alg}}    
%     \begin{tikzpicture}
%         \begin{pgfonlayer}{nodelayer}
%             \node [style=none] (122) at (1.875, -1) {};
%             \node [style=none] (123) at (1.875, 1) {};
%             \node [style=none] (124) at (-1.875, 1) {};
%             \node [style=none] (125) at (-1.875, -1) {};
%             \node [{dotStyle/+}] (128) at (-0.375, 0) {};
%             \node [style=none] (129) at (-1, 0) {};
%             \node [{dotStyle/-}] (131) at (-1.5, 0) {};
%             \node [{dotStyle/+}] (135) at (0.375, 0) {};
%             \node [style=none] (136) at (1, 0) {};
%             \node [{dotStyle/-}] (138) at (1.5, 0) {};
%             \node [style=none] (139) at (1, -0.475) {};
%             \node [style=none] (140) at (1, 0.475) {};
%             \node [style=none] (141) at (-1, 0.475) {};
%             \node [style=none] (142) at (-1, -0.475) {};
%         \end{pgfonlayer}
%         \begin{pgfonlayer}{edgelayer}
%             \draw [{bgStyle/-}] (124.center)
%                  to (123.center)
%                  to (122.center)
%                  to (125.center)
%                  to cycle;
%             \draw [{bgStyle/+}] (141.center)
%                  to (140.center)
%                  to (139.center)
%                  to (142.center)
%                  to cycle;
%             \draw [style={wStyle/+}] (135) to (136.center);
%             \draw [style={wStyle/+}] (128) to (129.center);
%             \draw [style={wStyle/-}] (138) to (136.center);
%             \draw [style={wStyle/-}] (129.center) to (131);
%         \end{pgfonlayer}
%     \end{tikzpicture}
%     \Leq{\text{Prop. }~\ref{prop:maps}}
%     \begin{tikzpicture}
%         \begin{pgfonlayer}{nodelayer}
%             \node [style=none] (122) at (1.875, -1) {};
%             \node [style=none] (123) at (1.875, 1) {};
%             \node [style=none] (124) at (-1.875, 1) {};
%             \node [style=none] (125) at (-1.875, -1) {};
%             \node [{dotStyle/-}] (128) at (-0.875, 0) {};
%             \node [style={dotStyle/-}] (129) at (-1.5, 0) {};
%             \node [{dotStyle/-}] (135) at (0.875, 0) {};
%             \node [{dotStyle/-}] (138) at (1.5, 0) {};
%             \node [style=none] (139) at (0.5, -0.475) {};
%             \node [style=none] (140) at (0.5, 0.475) {};
%             \node [style=none] (141) at (-0.5, 0.475) {};
%             \node [style=none] (142) at (-0.5, -0.475) {};
%         \end{pgfonlayer}
%         \begin{pgfonlayer}{edgelayer}
%             \draw [{bgStyle/-}] (124.center)
%                  to (123.center)
%                  to (122.center)
%                  to (125.center)
%                  to cycle;
%             \draw [{bgStyle/+}] (141.center)
%                  to (140.center)
%                  to (139.center)
%                  to (142.center)
%                  to cycle;
%             \draw [style={wStyle/-}] (128) to (129);
%             \draw [style={wStyle/-}] (135) to (138);
%         \end{pgfonlayer}
%     \end{tikzpicture}    
%     \Lgeq{\eqref{ax:minusCodiscDisc}}
%     \emptyCirc[+]
% \]

==> tikz/proofs/implication/notAorB.tex <==
\[ 
    \boxCirc[+]{a} 
    \Leq{\footnotesize{\stackanchor{\eqref{ax:comPlusUnit}}{\eqref{ax:monPlusUnit}}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{dotStyle/+}] (107) at (1, 0) {};
            \node [style=none] (108) at (0.4, 0.575) {};
            \node [style={dotStyle/+}] (109) at (0.4, -0.575) {};
            \node [style=none] (122) at (1.525, -1.2) {};
            \node [style=none] (123) at (1.525, 1.2) {};
            \node [style=none] (124) at (-1.5, 1.2) {};
            \node [style=none] (125) at (-1.5, -1.2) {};
            \node [style=none] (127) at (1.525, 0) {};
            \node [{dotStyle/+}] (128) at (-1, 0) {};
            \node [style=none] (129) at (-0.4, 0.575) {};
            \node [style={dotStyle/+}] (130) at (-0.4, -0.575) {};
            \node [style=none] (131) at (-1.5, 0) {};
            \node [style={boxStyle/+}] (134) at (0, 0.575) {$a$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{wStyle/+}, bend right=45] (109) to (107);
            \draw [{wStyle/+}, bend right=45] (107) to (108.center);
            \draw [{wStyle/+}] (107) to (127.center);
            \draw [{wStyle/+}, bend left=45] (130) to (128);
            \draw [{wStyle/+}, bend left=45] (128) to (129.center);
            \draw [{wStyle/+}] (128) to (131.center);
            \draw [style={wStyle/+}] (129.center) to (134);
            \draw [style={wStyle/+}] (134) to (108.center);
        \end{pgfonlayer}
    \end{tikzpicture}   
    \Lleq{(4)}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{dotStyle/+}] (107) at (2.4, 0.4) {};
            \node [style=none] (108) at (1.55, 1.325) {};
            \node [style=none] (109) at (1.55, -0.5) {};
            \node [style=none] (122) at (2.925, -1.95) {};
            \node [style=none] (123) at (2.925, 1.95) {};
            \node [style=none] (124) at (-2.825, 1.95) {};
            \node [style=none] (125) at (-2.825, -1.95) {};
            \node [style=none] (127) at (2.925, 0.4) {};
            \node [{dotStyle/+}] (128) at (-2.325, 0.375) {};
            \node [style=none] (129) at (-1.475, 1.325) {};
            \node [style=none] (130) at (-1.475, -0.5) {};
            \node [style=none] (131) at (-2.825, 0.375) {};
            \node [style={boxStyle/+}] (134) at (0, 1.325) {$a$};
            \node [{dotStyle/-}] (136) at (1.025, -0.5) {};
            \node [style=none] (137) at (0.425, 0.075) {};
            \node [style=none] (138) at (0.425, -1.075) {};
            \node [style=none] (139) at (1.55, -1.7) {};
            \node [style=none] (140) at (1.55, 0.7) {};
            \node [style=none] (141) at (-1.475, 0.7) {};
            \node [style=none] (142) at (-1.475, -1.7) {};
            \node [style=none] (143) at (1.55, -0.5) {};
            \node [{dotStyle/-}] (144) at (-0.975, -0.5) {};
            \node [style=none] (145) at (-0.375, 0.075) {};
            \node [style=none] (146) at (-0.375, -1.075) {};
            \node [style=none] (147) at (-1.475, -0.5) {};
            \node [style={boxStyle/-}] (149) at (0.025, 0.075) {${a}$};
            \node [style={boxStyle/+}] (150) at (0.025, -1.075) {$b$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{wStyle/+}, bend right=45] (109.center) to (107);
            \draw [{wStyle/+}, bend right=45] (107) to (108.center);
            \draw [{wStyle/+}] (107) to (127.center);
            \draw [{wStyle/+}, bend left=45] (130.center) to (128);
            \draw [{wStyle/+}, bend left=45] (128) to (129.center);
            \draw [{wStyle/+}] (128) to (131.center);
            \draw [style={wStyle/+}] (129.center) to (134);
            \draw [style={wStyle/+}] (134) to (108.center);
            \draw [{bgStyle/-}] (141.center)
                 to (140.center)
                 to (139.center)
                 to (142.center)
                 to cycle;
            \draw [{wStyle/-}, bend right=45] (138.center) to (136);
            \draw [{wStyle/-}, bend right=45] (136) to (137.center);
            \draw [{wStyle/-}] (136) to (143.center);
            \draw [{wStyle/-}, bend left=45] (146.center) to (144);
            \draw [{wStyle/-}, bend left=45] (144) to (145.center);
            \draw [{wStyle/-}] (144) to (147.center);
            \draw [style={wStyle/-}] (145.center) to (149);
            \draw [style={wStyle/-}] (146.center) to (150);
            \draw [style={wStyle/-}] (150) to (138.center);
            \draw [style={wStyle/-}] (149) to (137.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \stackrel{\footnotesize{\stackanchor{Lemma}{\ref{lm:linearly distr cat}.3}}}{\leq}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{dotStyle/-}] (107) at (2.4, -0.4) {};
            \node [style=none] (108) at (1.55, -1.325) {};
            \node [style=none] (109) at (1.55, 0.5) {};
            \node [style=none] (122) at (2.925, 1.95) {};
            \node [style=none] (123) at (2.925, -1.95) {};
            \node [style=none] (124) at (-2.825, -1.95) {};
            \node [style=none] (125) at (-2.825, 1.95) {};
            \node [style=none] (127) at (2.925, -0.4) {};
            \node [{dotStyle/-}] (128) at (-2.325, -0.375) {};
            \node [style=none] (129) at (-1.475, -1.325) {};
            \node [style=none] (130) at (-1.475, 0.5) {};
            \node [style=none] (131) at (-2.825, -0.375) {};
            \node [style={boxStyle/+}] (134) at (0, -1.325) {$b$};
            \node [{dotStyle/+}] (136) at (1.025, 0.5) {};
            \node [style=none] (137) at (0.425, -0.075) {};
            \node [style=none] (138) at (0.425, 1.075) {};
            \node [style=none] (139) at (1.55, 1.7) {};
            \node [style=none] (140) at (1.55, -0.7) {};
            \node [style=none] (141) at (-1.475, -0.7) {};
            \node [style=none] (142) at (-1.475, 1.7) {};
            \node [style=none] (143) at (1.55, 0.5) {};
            \node [{dotStyle/+}] (144) at (-0.975, 0.5) {};
            \node [style=none] (145) at (-0.375, -0.075) {};
            \node [style=none] (146) at (-0.375, 1.075) {};
            \node [style=none] (147) at (-1.475, 0.5) {};
            \node [style={boxStyle/-}] (149) at (0.025, -0.075) {${a}$};
            \node [style={boxStyle/+}] (150) at (0.025, 1.075) {$a$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{wStyle/-}, bend left=45] (109.center) to (107);
            \draw [{wStyle/-}, bend left=45] (107) to (108.center);
            \draw [{wStyle/-}] (107) to (127.center);
            \draw [{wStyle/-}, bend right=45] (130.center) to (128);
            \draw [{wStyle/-}, bend right=45] (128) to (129.center);
            \draw [{wStyle/-}] (128) to (131.center);
            \draw [style={wStyle/-}] (129.center) to (134);
            \draw [style={wStyle/-}] (134) to (108.center);
            \draw [{bgStyle/+}] (141.center)
                 to (140.center)
                 to (139.center)
                 to (142.center)
                 to cycle;
            \draw [{wStyle/+}, bend left=45] (138.center) to (136);
            \draw [{wStyle/+}, bend left=45] (136) to (137.center);
            \draw [{wStyle/+}] (136) to (143.center);
            \draw [{wStyle/+}, bend right=45] (146.center) to (144);
            \draw [{wStyle/+}, bend right=45] (144) to (145.center);
            \draw [{wStyle/+}] (144) to (147.center);
            \draw [style={wStyle/+}] (145.center) to (149);
            \draw [style={wStyle/+}] (146.center) to (150);
            \draw [style={wStyle/+}] (150) to (138.center);
            \draw [style={wStyle/+}] (149) to (137.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \stackrel{\footnotesize{\stackanchor{Table}{\ref{table:daggerrlalattice}}}}{=}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{dotStyle/-}] (107) at (1, 0) {};
            \node [style=none] (108) at (0.4, -0.575) {};
            \node [style={dotStyle/-}] (109) at (0.4, 0.575) {};
            \node [style=none] (122) at (1.525, 1.2) {};
            \node [style=none] (123) at (1.525, -1.2) {};
            \node [style=none] (124) at (-1.5, -1.2) {};
            \node [style=none] (125) at (-1.5, 1.2) {};
            \node [style=none] (127) at (1.525, 0) {};
            \node [{dotStyle/-}] (128) at (-1, 0) {};
            \node [style=none] (129) at (-0.4, -0.575) {};
            \node [style={dotStyle/-}] (130) at (-0.4, 0.575) {};
            \node [style=none] (131) at (-1.5, 0) {};
            \node [style={boxStyle/+}] (134) at (0, -0.575) {$b$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{wStyle/-}, bend left=45] (109) to (107);
            \draw [{wStyle/-}, bend left=45] (107) to (108.center);
            \draw [{wStyle/-}] (107) to (127.center);
            \draw [{wStyle/-}, bend right=45] (130) to (128);
            \draw [{wStyle/-}, bend right=45] (128) to (129.center);
            \draw [{wStyle/-}] (128) to (131.center);
            \draw [style={wStyle/-}] (129.center) to (134);
            \draw [style={wStyle/-}] (134) to (108.center);
        \end{pgfonlayer}
    \end{tikzpicture}   
    \Leq{\footnotesize{\stackanchor{\eqref{ax:comMinusUnit}}{\eqref{ax:monMinusUnit}}}}
    \boxCirc[+]{b}
\]

==> tikz/proofs/phiLemma.tex <==
The proof goes by induction on the rules in~\eqref{eq:pc}.

For the rule $(id)$ we have three cases: either $(c,d) \in \T{I}$ or $(c,d) \in \syninclusionT{\sign'}$ or $(c,d) \in \TMAP{k}$. If $(c,d) \in \T{I}$ then, by Lemma~\ref{lm:phi characterization}, $\phi(c) = \phiCirc[+]{c} \syninclusionT{\T{T}} \phiCirc[+]{d} = \phi(d)$.

If $(c,d) \in \syninclusionT{\sign'}$ then $(c,d)$ has been obtained by instantiating the axioms in Figures~\ref{fig:cb axioms},\ref{fig:cocb axioms} and \ref{fig:closed lin axioms} with diagrams containing $k$. Therefore, we need to show that $\phi$ preserves these axioms. In the following we show only $\eqref{ax:comPlusLaxNat}, \eqref{ax:discPlusLaxNat}, \eqref{ax:leftLinDistr}$, $\eqref{ax:linStrn2}$, $\eqref{ax:tauRPlus}$ and $\eqref{ax:gammaRPlus}$. The remaining ones follow similar reasonings.
\input{tikz/proofs/phiLemma/copier.tex}
% \begin{figure}[H]
%     \centering
%     \includegraphics*[scale=0.45]{pdf_proofs/phiCopier.pdf}
% \end{figure}

\input{tikz/proofs/phiLemma/discard.tex}
% \begin{figure}[H]
%     \centering
%     \includegraphics*[scale=0.45]{pdf_proofs/phiDiscard.pdf}
% \end{figure}

\input{tikz/proofs/phiLemma/linDistr.tex}
% \begin{figure}[H]
%     \centering
%     \includegraphics*[scale=0.45]{pdf_proofs/phiDistr.pdf}
% \end{figure}

% \marginpar{Refer to the spider theorem in the step marked with $(\ast)$. maybe in a footnote}
\input{tikz/proofs/phiLemma/linStr.tex}
% \begin{figure}[H]
%     \centering
%     \includegraphics*[scale=0.45]{pdf_proofs/phiLinStr.pdf}
% \end{figure}

\input{tikz/proofs/phiLemma/linAdjRel.tex}

Similar to the previous argument, if $(c,d) \in \TMAP{k}$ then it is enough to show that $\phi$ preserves the axioms in $\TMAP{k}$.

\input{tikz/proofs/phiLemma/copierK.tex}

\input{tikz/proofs/phiLemma/discardK.tex}

The base case $(r)$ is trivial, while the proof for the remaining rules follows a straightforward inductive argument.

==> tikz/remarkContr.tex <==
\begin{equation}\label{eq:remcounter}
    \emptyCirc[+] \stackrel{\eqref{eq:bone}}{\syninclusionT{\T{T}}} \tikzfig{axioms/cb/plus/codiscDisc} \stackrel{(tr)}{\syninclusionT{\T{T}}} \tikzfig{axioms/linadj/cobangPbang} \stackrel{\eqref{ax:gammaDiscardPlus}}{\syninclusionT{\T{T}}} \emptyCirc[-]
\end{equation}

==> tikz/wrongway/statement.tex <==
\[
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{boxStyle/+}] (134) at (0.5, 0.5) {$c$};
            \node [style=none] (135) at (-1.25, 0) {};
            \node [style=none] (136) at (-1.25, 1.225) {};
            \node [style=none] (137) at (-1.25, -1) {};
            \node [style=none] (138) at (1.25, -1) {};
            \node [style=none] (139) at (1.25, 1.225) {};
            \node [style={dotStyle/+}] (144) at (-0.5, 0) {};
            \node [style=none] (145) at (0.25, -0.5) {};
            \node [style=none] (146) at (1.25, 0.5) {};
            \node [style=none] (147) at (1.25, -0.5) {};
            \node [style=none] (150) at (0.25, 0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (138.center)
                 to (137.center)
                 to (136.center)
                 to (139.center)
                 to cycle;
            \draw [style={wStyle/+}, bend left] (145.center) to (144);
            \draw [style={wStyle/+}] (144) to (135.center);
            \draw [style={wStyle/+}] (134) to (146.center);
            \draw [style={wStyle/+}] (147.center) to (145.center);
            \draw [style={wStyle/+}] (134) to (150.center);
            \draw [style={wStyle/+}, bend right] (150.center) to (144);
        \end{pgfonlayer}
    \end{tikzpicture}
    \leq
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{boxOpStyle/+}] (134) at (-1, -0.25) {$c$};
            \node [style={boxStyle/+}] (135) at (-3, 0.25) {$c$};
            \node [style=none] (136) at (-3.75, 1.225) {};
            \node [style=none] (137) at (-3.75, -1) {};
            \node [style=none] (138) at (-0.25, -1) {};
            \node [style=none] (139) at (-0.25, 1.225) {};
            \node [style={dotStyle/+}] (144) at (-2, 0.25) {};
            \node [style=none] (145) at (-1.25, 0.75) {};
            \node [style=none] (146) at (-0.25, 0.75) {};
            \node [style=none] (147) at (-0.25, -0.25) {};
            \node [style=none] (150) at (-1.25, -0.25) {};
            \node [style=none] (152) at (-3.75, 0.25) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (138.center)
                 to (137.center)
                 to (136.center)
                 to (139.center)
                 to cycle;
            \draw [style={wStyle/+}, bend right] (145.center) to (144);
            \draw [style={wStyle/+}] (144) to (135);
            \draw [style={wStyle/+}] (134) to (150.center);
            \draw [style={wStyle/+}, bend left] (150.center) to (144);
            \draw [style={wStyle/+}] (134) to (147.center);
            \draw [style={wStyle/+}] (146.center) to (145.center);
            \draw [style={wStyle/+}] (135) to (152.center);
        \end{pgfonlayer}
    \end{tikzpicture}        
    \qquad\qquad
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{boxOpStyle/+}] (134) at (-1, -0.25) {$c$};
            \node [style={boxStyle/+}] (135) at (-3, 0.25) {$c$};
            \node [style=none] (136) at (-3.75, 1.225) {};
            \node [style=none] (137) at (-3.75, -1) {};
            \node [style=none] (138) at (-0.25, -1) {};
            \node [style=none] (139) at (-0.25, 1.225) {};
            \node [style={dotStyle/-}] (144) at (-2, 0.25) {};
            \node [style=none] (145) at (-1.25, 0.75) {};
            \node [style=none] (146) at (-0.25, 0.75) {};
            \node [style=none] (147) at (-0.25, -0.25) {};
            \node [style=none] (150) at (-1.25, -0.25) {};
            \node [style=none] (152) at (-3.75, 0.25) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (138.center)
                 to (137.center)
                 to (136.center)
                 to (139.center)
                 to cycle;
            \draw [style={wStyle/-}, bend right] (145.center) to (144);
            \draw [style={wStyle/-}] (144) to (135);
            \draw [style={wStyle/-}] (134) to (150.center);
            \draw [style={wStyle/-}, bend left] (150.center) to (144);
            \draw [style={wStyle/-}] (134) to (147.center);
            \draw [style={wStyle/-}] (146.center) to (145.center);
            \draw [style={wStyle/-}] (135) to (152.center);
        \end{pgfonlayer}
    \end{tikzpicture}   
    \leq
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [{boxStyle/+}] (134) at (0.5, 0.5) {$c$};
            \node [style=none] (135) at (-1.25, 0) {};
            \node [style=none] (136) at (-1.25, 1.225) {};
            \node [style=none] (137) at (-1.25, -1) {};
            \node [style=none] (138) at (1.25, -1) {};
            \node [style=none] (139) at (1.25, 1.225) {};
            \node [style={dotStyle/-}] (144) at (-0.5, 0) {};
            \node [style=none] (145) at (0.25, -0.5) {};
            \node [style=none] (146) at (1.25, 0.5) {};
            \node [style=none] (147) at (1.25, -0.5) {};
            \node [style=none] (150) at (0.25, 0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (138.center)
                 to (137.center)
                 to (136.center)
                 to (139.center)
                 to cycle;
            \draw [style={wStyle/-}, bend left] (145.center) to (144);
            \draw [style={wStyle/-}] (144) to (135.center);
            \draw [style={wStyle/-}] (134) to (146.center);
            \draw [style={wStyle/-}] (147.center) to (145.center);
            \draw [style={wStyle/-}] (134) to (150.center);
            \draw [style={wStyle/-}, bend right] (150.center) to (144);
        \end{pgfonlayer}
    \end{tikzpicture} 
\]
